Overinference from Weak Signals and Underinference from Strong Signals

When people receive new information, sometimes they revise their beliefs too much, and sometimes too little. In this paper, we show that a key driver of whether people overinfer or underinfer is the strength of the information. Based on a model in which people know which direction to update in, but not exactly how much to update, we hypothesize that people will overinfer from weak signals and underinfer from strong signals. We then test this hypothesis across four different environments: abstract experiments, a naturalistic experiment, sports betting markets, and financial markets. In each environment, our consistent and robust finding is overinference from weak signals and underinference from strong signals. Our framework and findings can help harmonize apparently contradictory results from the experimental and empirical literatures.

==> experiment/abstract2_quantile_results.tex <==
\begin{tabular}{l*{5}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                              &\multicolumn{1}{c}{10th}&\multicolumn{1}{c}{30th}&\multicolumn{1}{c}{50th}&\multicolumn{1}{c}{70th}&\multicolumn{1}{c}{90th}\\
\hline
Signal Strength               &    0.178&   -0.133&   -0.160&   -0.661&   -1.724\\
                              &  (0.056)&  (0.012)&  (0.037)&  (0.034)&  (0.034)\\
\hline
Observations                  &     2500&     2500&     2500&     2500&     2500\\
\hline\hline
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> experiment/grether_replication.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                              &\multicolumn{1}{c}{50\% Prior}&\multicolumn{1}{c}{All Priors}&\multicolumn{1}{c}{All Priors}&\multicolumn{1}{c}{All Priors}\\
\hline
Signal Strength: 0.05         &    2.371&    2.844&    2.800&    2.795\\
                              &  (0.224)&  (0.286)&  (0.179)&  (0.178)\\
Signal Strength: 0.20         &    1.359&    1.554&    1.504&    1.500\\
                              &  (0.072)&  (0.083)&  (0.059)&  (0.059)\\
Signal Strength: 0.50         &    1.176&    1.208&    1.190&    1.191\\
                              &  (0.054)&  (0.041)&  (0.035)&  (0.035)\\
Signal Strength: 1.25         &    0.840&    0.852&    0.857&    0.857\\
                              &  (0.028)&  (0.021)&  (0.020)&  (0.020)\\
Signal Strength: 1.75         &    0.824&    0.768&    0.762&    0.762\\
                              &  (0.021)&  (0.017)&  (0.015)&  (0.015)\\
Logit Prior                   &         &         &    0.984&         \\
                              &         &         &  (0.016)&         \\
Logit Prior: Signal=0.05      &         &         &         &    1.028\\
                              &         &         &         &  (0.017)\\
Logit Prior: Signal=0.20      &         &         &         &    1.036\\
                              &         &         &         &  (0.021)\\
Logit Prior: Signal=0.50      &         &         &         &    0.996\\
                              &         &         &         &  (0.023)\\
Logit Prior: Signal=1.25      &         &         &         &    0.944\\
                              &         &         &         &  (0.029)\\
Logit Prior: Signal=1.75      &         &         &         &    0.915\\
                              &         &         &         &  (0.029)\\
Subject FE                    &      Yes&      Yes&      Yes&      Yes\\
Round FE                      &      Yes&      Yes&      Yes&      Yes\\
\hline
Observations                  &     2500&     7500&     7500&     7500\\
\(R^{2}\)                     &     0.80&     0.60&     0.76&     0.76\\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> experiment/heterogeneity_main.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                              &\multicolumn{1}{c}{By Variance}&\multicolumn{1}{c}{By SD of Weights}&\multicolumn{1}{c}{By CRT Score}&\multicolumn{1}{c}{By News}\\
\hline
Signal Strength               &    0.118&   -0.072&   -0.175&   -0.185\\
                              &  (0.031)&  (0.051)&  (0.040)&  (0.050)\\
Strength x SD of Weights      &   -0.383&         &         &         \\
                              &  (0.036)&         &         &         \\
Strength x Round Num          &         &   -0.042&         &         \\
                              &         &  (0.009)&         &         \\
Strength x CRT Qs incorrect   &         &         &   -0.102&         \\
                              &         &         &  (0.028)&         \\
Strength x Less News          &         &         &         &   -0.334\\
                              &         &         &         &  (0.129)\\
Constant                      &    1.395&    1.416&    1.421&    1.420\\
                              &  (0.021)&  (0.030)&  (0.030)&  (0.030)\\
Subject FE                    &      Yes&      Yes&      Yes&      Yes\\
Round FE                      &      Yes&      Yes&      Yes&      Yes\\
\hline
Observations                  &     3962&     3964&     3964&     3964\\
\(R^{2}\)                     &     0.28&     0.24&     0.23&     0.23\\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> experiment/heterogeneity_replication.tex <==
\begin{tabular}{l*{3}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                              &\multicolumn{1}{c}{By SD of Weights}&\multicolumn{1}{c}{By Round}&\multicolumn{1}{c}{By Uncertainty}\\
\hline
Weight on Prior               &   -0.020&   -0.020&   -0.020\\
                              &  (0.013)&  (0.013)&  (0.013)\\
Signal Strength               &   -0.002&   -0.698&   -0.756\\
                              &  (0.070)&  (0.089)&  (0.120)\\
Strength x SD of Weights      &   -0.433&         &         \\
                              &  (0.046)&         &         \\
Strength x Round Num          &         &   -0.037&         \\
                              &         &  (0.012)&         \\
Strength x Uncertain          &         &         &   -0.542\\
                              &         &         &  (0.288)\\
Constant                      &    2.147&    2.183&    2.181\\
                              &  (0.037)&  (0.048)&  (0.048)\\
Subject FE                    &      Yes&      Yes&      Yes\\
Round FE                      &      Yes&      Yes&      Yes\\
\hline
Observations                  &     7500&     7500&     7500\\
\(R^{2}\)                     &     0.20&     0.17&     0.17\\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> experiment/linear_results.tex <==
\begin{tabular}{l*{5}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                              &\multicolumn{1}{c}{Main Effects}&\multicolumn{1}{c}{By Noise}&\multicolumn{1}{c}{By Round}&\multicolumn{1}{c}{By CRT Score}&\multicolumn{1}{c}{By News}\\
\hline
Signal Strength               &   -0.308&    0.118&   -0.072&   -0.175&   -0.185\\
                              &  (0.031)&  (0.031)&  (0.051)&  (0.040)&  (0.050)\\
Strength x SD of Weights      &         &   -0.383&         &         &         \\
                              &         &  (0.036)&         &         &         \\
Strength x Round Num          &         &         &   -0.042&         &         \\
                              &         &         &  (0.009)&         &         \\
Strength x CRT Qs incorrect   &         &         &         &   -0.102&         \\
                              &         &         &         &  (0.028)&         \\
Strength x Less News          &         &         &         &         &   -0.334\\
                              &         &         &         &         &  (0.129)\\
Constant                      &    1.420&    1.395&    1.416&    1.421&    1.420\\
                              &  (0.030)&  (0.021)&  (0.030)&  (0.030)&  (0.030)\\
Subject FE                    &      Yes&      Yes&      Yes&      Yes&      Yes\\
Round FE                      &      Yes&      Yes&      Yes&      Yes&      Yes\\
\hline
Observations                  &     3964&     3962&     3964&     3964&     3964\\
\(R^{2}\)                     &     0.23&     0.28&     0.24&     0.23&     0.23\\
\hline\hline
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> experiment/linear_results_abstract2.tex <==
\begin{tabular}{l*{5}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                              &\multicolumn{1}{c}{50\% Prior}&\multicolumn{1}{c}{All Priors}&\multicolumn{1}{c}{By SD of Weights}&\multicolumn{1}{c}{By Round}&\multicolumn{1}{c}{By Confidence}\\
\hline
Signal Strength               &   -0.624&   -0.942&   -0.041&   -1.237&   -1.320\\
                              &  (0.048)&  (0.065)&  (0.079)&  (0.127)&  (0.201)\\
Strength x SD of Weights      &         &         &   -0.413&         &         \\
                              &         &         &  (0.053)&         &         \\
Strength x Round Number       &         &         &         &    0.037&         \\
                              &         &         &         &  (0.012)&         \\
Average Confidence            &         &         &         &         &   -0.006\\
                              &         &         &         &         &  (0.004)\\
Strength x Confidence         &         &         &         &         &    0.006\\
                              &         &         &         &         &  (0.003)\\
Constant                      &    1.768&    2.157&    2.125&    2.158&    2.548\\
                              &  (0.036)&  (0.049)&  (0.038)&  (0.049)&  (0.289)\\
Subject FE                    &      Yes&      Yes&      Yes&      Yes&       No\\
Round FE                      &      Yes&      Yes&      Yes&      Yes&      Yes\\
\hline
Observations                  &     2492&     7456&     7456&     7456&     7456\\
\(R^{2}\)                     &     0.41&     0.16&     0.19&     0.16&     0.05\\
\hline\hline
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> experiment/linear_results_grether.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                              &\multicolumn{1}{c}{50\% Prior}&\multicolumn{1}{c}{Non-50\% Prior}&\multicolumn{1}{c}{All Priors}&\multicolumn{1}{c}{All Priors}\\
\hline
Weak x Signal Strength        &    1.410&    1.615&    1.581&    1.577\\
                              &  (0.077)&  (0.089)&  (0.060)&  (0.060)\\
Strong x Signal Strength      &    0.830&    0.775&    0.794&    0.794\\
                              &  (0.018)&  (0.017)&  (0.015)&  (0.015)\\
Logit Prior                   &         &         &    0.969&         \\
                              &         &         &  (0.018)&         \\
Weak x Logit Prior            &         &         &         &    1.021\\
                              &         &         &         &  (0.018)\\
Strong x Logit Prior          &         &         &         &    0.916\\
                              &         &         &         &  (0.024)\\
Subject FE                    &      Yes&      Yes&      Yes&      Yes\\
Round FE                      &      Yes&      Yes&      Yes&      Yes\\
\hline
Observations                  &     2008&     4007&     6015&     6015\\
\(R^{2}\)                     &     0.83&     0.70&     0.77&     0.77\\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> experiment/linear_results_may2024.tex <==
\begin{tabular}{l*{5}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                              &\multicolumn{1}{c}{Main Effects}&\multicolumn{1}{c}{By Noise}&\multicolumn{1}{c}{By Round}&\multicolumn{1}{c}{By CRT Score}&\multicolumn{1}{c}{By News}\\
\hline
Signal Strength               &   -0.308&   -0.145&   -0.578&   -0.481&   -0.519\\
                              &  (0.031)&  (0.059)&  (0.072)&  (0.064)&  (0.093)\\
Strength x Noise Percentile   &         &   -0.349&         &         &         \\
                              &         &  (0.138)&         &         &         \\
Strength x Round Number       &         &         &    0.042&         &         \\
                              &         &         &  (0.009)&         &         \\
Strength x CRT Score          &         &         &         &    0.102&         \\
                              &         &         &         &  (0.028)&         \\
Strength x News Cons          &         &         &         &         &    0.334\\
                              &         &         &         &         &  (0.129)\\
Constant                      &    1.420&    1.404&    1.416&    1.421&    1.420\\
                              &  (0.030)&  (0.042)&  (0.030)&  (0.030)&  (0.030)\\
Subject FE                    &      Yes&      Yes&      Yes&      Yes&      Yes\\
Round FE                      &      Yes&      Yes&      Yes&      Yes&      Yes\\
\hline
Observations                  &     3964&     1901&     3964&     3964&     3964\\
\(R^{2}\)                     &     0.23&     0.29&     0.24&     0.23&     0.23\\
\hline\hline
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> experiment/linear_results_nba.tex <==
\begin{tabular}{l*{3}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                              &\multicolumn{1}{c}{Both Halves}&\multicolumn{1}{c}{Both Halves}&\multicolumn{1}{c}{Both Halves}\\
\hline
1st Half x Signal Strength    &    1.375&    1.375&    1.374\\
                              &  (0.083)&  (0.050)&  (0.050)\\
2nd Half x Signal Strength    &    0.755&    0.614&    0.616\\
                              &  (0.034)&  (0.019)&  (0.019)\\
Logit Prior                   &         &    0.905&         \\
                              &         &  (0.013)&         \\
1st Half x Logit Prior        &         &         &    0.968\\
                              &         &         &  (0.029)\\
2nd Half x Logit Prior        &         &         &    0.892\\
                              &         &         &  (0.013)\\
Subject FE                    &      Yes&      Yes&      Yes\\
Round FE                      &      Yes&      Yes&      Yes\\
Quarter FE                    &      Yes&      Yes&      Yes\\
\hline
Observations                  &     8000&     8000&     8000\\
\(R^{2}\)                     &     0.48&     0.86&     0.86\\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> experiment/linear_results_ned_messing_around.tex <==
\begin{tabular}{l 
cc!{\color{gray!30}\vrule width 0.3pt} 
cc!{\color{gray!30}\vrule width 0.3pt} 
cc}
\toprule

  DV: Weight on signal
  &\multicolumn{2}{c!{\color{gray!30}\vrule width 0.3pt}}{Study 1a} 
  & \multicolumn{2}{c!{\color{gray!30}\vrule width 0.3pt}}{Study 1b} 
  & \multicolumn{2}{c}{Study 2} \\

 \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
  
  &\multicolumn{1}{c}{(1)}
  &\multicolumn{1}{c!{\color{gray!30}\vrule width 0.3pt}}{(2)}
  &\multicolumn{1}{c}{(3)}
  &\multicolumn{1}{c!{\color{gray!30}\vrule width 0.3pt}}{(4)}
  &\multicolumn{1}{c}{(5)}
  &\multicolumn{1}{c}{(6)}\\


\hline

Constant             & 1.420   &  & 2.182 & & 1.700 & \\
                      & (0.030) &  & (0.048) & & (0.025) & \\
Signal Strength       & -0.308  &  & -0.958 & & -2.060 & \\
                      & (0.031) &  & (0.065) & & (0.112) & \\
Structural: $\beta$       & & 0.761 &  & 0.605 & & 0.285 \\
                      & & (0.028) &  & (0.022) & & (0.041) \\
Structural: $k$         & & 0.883 &  & 0.887 & & 0.305 \\
                      & & (0.023) &  & (0.022) & & (0.026) \\
Weight on Prior ($\alpha$)  & -  & - &              0.980&   0.978&   0.976 &   0.971\\
                            &  - & - &              (0.013)&  (0.013)&  (0.009) &  (0.010)\\
                    
\rule{0pt}{4ex}Subject FE                    &      Yes&      No&      Yes&      No&      Yes &      No\\
Round FE                      &      Yes&      No&      Yes&      No&      Yes &      No\\
\hline
Observations                  &     3964&     3964&     7500&     7500&     8000 &     8000\\
\(R^{2}\)                     &     0.23&     0.38&     0.17&     0.26&     0.24 &     0.36\\
\bottomrule
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}



==> experiment/linear_results_ned_messing_around2Old.tex <==
\begin{tabular}{l cccc!{\color{gray!30}\vrule width 0.3pt} ccc}
\toprule

DV: Weight on Signal  &\multicolumn{4}{c!{\color{gray!30}\vrule width 0.3pt}}{Study 1a} & \multicolumn{3}{c}{Study 1b} \\

% &\multicolumn{4}{c!{\color{gray!30}\vrule width 0.3pt}}{(Abstract)} & \multicolumn{3}{c}{(Vary Priors)} \\

  

\cmidrule(lr){2-5} \cmidrule(lr){6-8} 

  &\multicolumn{1}{c}{(1)}
  &\multicolumn{1}{c}{(2)}
  &\multicolumn{1}{c}{(3)}
  &\multicolumn{1}{c!{\color{gray!30}\vrule width 0.3pt}}{(4)}
  &\multicolumn{1}{c}{(5)}
  &\multicolumn{1}{c}{(6)}
  &\multicolumn{1}{c}{(7)} \\

\hline

Constant   &   1.395&    1.416&   1.421&   1.420&   2.147 &   2.183 & 2.181 \\
                              &  (0.021)&  (0.030)&  (0.030)&  (0.030)&  (0.037) &  (0.048) & (0.048) \\
Strength          &   0.118&    -0.072&   -0.175&   -0.185&   -0.002 &   -0.698 &   -0.756\\
                              &  (0.036)&  (0.009)&  (0.028)&  (0.129)&  (0.070) &  (0.089) &  (0.120)\\    
\hspace{3mm}  Strength $\times$ Noise        
& -0.383  & & & & -0.433 & &  \\
& (0.036)  & & & & (0.046) & &  \\               
\hspace{3mm}  Strength $\times$ Inexperience   
& & -0.042 & & & & -0.037 &  \\
& & (0.009) & & & & (0.012) &  \\                 
\hspace{3mm}  Strength $\times$ CRT incorrect       
& & & -0.102 & & & &  \\
& & & (0.028) & & & &  \\  
\hspace{3mm}  Strength $\times$ Less News        
& & & & -0.334  & & &  \\
& & & & (0.129)  & & &  \\  
\hspace{3mm}  Strength $\times$ Uncertainty
& & & & & & & -0.542 \\
& & & & & & & (0.288) \\   
Weight on Prior         &   &   &   &   & 0.980 &  0.980  & 0.980  \\
                              &  &  &  &  &  (0.013) &  (0.013) &  (0.013)\\    
\rule{0pt}{4ex}Subject FE                    &      Yes&      Yes&      Yes&      Yes&      Yes &      Yes  &      Yes\\
Round FE                      &      Yes&      Yes&      Yes&      Yes&      Yes &      Yes &      Yes\\
\hline
Observations                  &     3964&     3962&     3964&     3962&     7500 &     7500 &     7500\\
\(R^{2}\)                     &     0.28&     0.24&     0.23&     0.23&     0.20 &     0.17 &     0.17\\
\bottomrule
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}



==> experiment/linear_results_ned_messing_around3.tex <==
\begin{tabular}{l 
cc 
cc 
cc}
\toprule

  DV: Weight on signal

  &\multicolumn{3}{c}{Regression} 
  & \multicolumn{3}{c}{Structural} \\

 \cmidrule(lr){2-4} \cmidrule(lr){5-7}  
  
  &\multicolumn{1}{c}{Study 1a}
  & \multicolumn{1}{c}{Study 1b} 
  & \multicolumn{1}{c}{Study 2}
  &\multicolumn{1}{c}{Study 1a}
  & \multicolumn{1}{c}{Study 1b} 
  & \multicolumn{1}{c}{Study 2} \\
  

\hline

Constant             & 1.42   &  2.13? & 1.42? & & & \\
                      & (0.03) & (?) & (?) & & & \\
Signal Strength       & -0.31   & -0.53? & -0.23? & & & \\
                      & (0.03)  & (?) & (?) & & & \\
Structural: $\beta$      & & & & 0.76 &  0.61 & 0.30 \\
                      & & & & (?)  & (?) & (?) \\
Structural: $k$         & & & & ? &  ? & ? \\
                      & & & & (?)  & (?) & (?) \\
\rule{0pt}{4ex}Base-Rate Neglect ($\alpha$)  & -  &      0.92&   0.91&  - & 0.85 &   0.82\\
                            &  - &               (0.07)&  (0.06)& - & (0.09) &  (0.09)\\
                    
\rule{0pt}{4ex}Subject FE                    &      Yes&      Yes&      Yes&      Yes&      Yes &      Yes\\
Round FE                      &      Yes&      Yes&      Yes&      Yes&      Yes &      Yes\\
\hline
Observations                  &     3964&     7456&   8000 &     3964&     7456&   8000 \\
\(R^{2}\)                     &     0.23&     0.28&     0.24&     0.23&     0.23 &     0.23\\
\bottomrule
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}



==> experiment/linear_results_ned_messing_around5.tex <==
\begin{tabular}{l 
c!{\color{gray!30}\vrule width 0.3pt} 
cc!{\color{gray!30}\vrule width 0.3pt} 
cc}
\toprule

  DV: Weight on signal
  &\multicolumn{1}{c!{\color{gray!30}\vrule width 0.3pt}}{Study 1a} 
  & \multicolumn{2}{c!{\color{gray!30}\vrule width 0.3pt}}{Study 1b} 
  & \multicolumn{2}{c}{Study 2} \\

 \cmidrule(lr){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}

  
  &\multicolumn{1}{c!{\color{gray!30}\vrule width 0.3pt}}{(1)}
  &\multicolumn{1}{c}{(2)}
  &\multicolumn{1}{c!{\color{gray!30}\vrule width 0.3pt}}{(3)}
  &\multicolumn{1}{c}{(4)}
  &\multicolumn{1}{c}{(5)}\\


\hline

Constant             & 1.420   & 1.768 & 2.182 & ? & 1.700 \\
                      & (0.030) & (0.036) & (0.048) & ? & (0.025)  \\
Signal Strength       & -0.308  & -0.624 & -0.958 & ?  & -2.060 \\
                      & (0.031) & (0.048) & (0.065) & ?  & (0.112) \\
Estimated Prior Weight ($\alpha$)  &   &  &  0.980&  & 0.976\\
                            &   &  &   (0.013)& &  (0.009)\\
                    
\rule{0pt}{4ex}Subject FE                    &      Yes&      Yes&      Yes&     Yes &      Yes\\
Round FE                      &      Yes&      Yes&      Yes&      Yes&      Yes \\
\hline
Observations                  &     3964&     7500&     7500&     8000 &     8000\\
\(R^{2}\)                     &     0.23&     0.17&     0.26&     0.24 &     0.36\\
\bottomrule
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}




==> experiment/quantile_results.tex <==
\begin{tabular}{l*{5}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                              &\multicolumn{1}{c}{10th}&\multicolumn{1}{c}{30th}&\multicolumn{1}{c}{50th}&\multicolumn{1}{c}{70th}&\multicolumn{1}{c}{90th}\\
\hline
Signal Strength               &    0.130&   -0.027&   -0.018&   -0.187&   -0.612\\
                              &  (0.041)&  (0.012)&  (0.005)&  (0.016)&  (0.055)\\
\hline
Observations                  &     3964&     3964&     3964&     3964&     3964\\
\hline\hline
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> experiment/weights_nba.tex <==
\begin{tabular}{l*{2}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                              &\multicolumn{1}{c}{50\% Prior}&\multicolumn{1}{c}{All Priors}\\
\hline
Signal Strength               &   -2.078&   -2.060\\
                              &  (0.111)&  (0.112)\\
Weight on Prior               &         &   -0.024\\
                              &         &  (0.009)\\
Constant                      &    1.706&    1.700\\
                              &  (0.024)&  (0.025)\\
Subject FE                    &      Yes&      Yes\\
Round FE                      &      Yes&      Yes\\
\hline
Observations                  &     8000&     8000\\
\(R^{2}\)                     &     0.24&     0.24\\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> experiment/weights_replication_main.tex <==
\begin{tabular}{l*{3}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                              &\multicolumn{1}{c}{50\% Prior}&\multicolumn{1}{c}{All Priors}&\multicolumn{1}{c}{All Priors}\\
\hline
Signal Strength               &   -0.637&   -0.957&   -0.958\\
                              &  (0.048)&  (0.065)&  (0.065)\\
Weight on Prior               &         &         &   -0.020\\
                              &         &         &  (0.013)\\
Constant                      &    1.787&    2.180&    2.182\\
                              &  (0.036)&  (0.049)&  (0.048)\\
Subject FE                    &      Yes&      Yes&      Yes\\
Round FE                      &      Yes&      Yes&      Yes\\
\hline
Observations                  &     2500&     7500&     7500\\
\(R^{2}\)                     &     0.41&     0.16&     0.17\\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> linear_results_abstract2.tex <==
\begin{tabular}{l*{5}{c}}
\hline\hline
                              &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                              &\multicolumn{1}{c}{50\% Prior}&\multicolumn{1}{c}{All Priors}&\multicolumn{1}{c}{By SD of Weights}&\multicolumn{1}{c}{By Round}&\multicolumn{1}{c}{By Confidence}\\
\hline
Signal Strength               &   -0.624&   -0.942&   -0.041&   -1.237&   -1.320\\
                              &  (0.048)&  (0.065)&  (0.079)&  (0.127)&  (0.201)\\
Strength x SD of Weights      &         &         &   -0.413&         &         \\
                              &         &         &  (0.053)&         &         \\
Strength x Round Number       &         &         &         &    0.037&         \\
                              &         &         &         &  (0.012)&         \\
Average Confidence            &         &         &         &         &   -0.006\\
                              &         &         &         &         &  (0.004)\\
Strength x Confidence         &         &         &         &         &    0.006\\
                              &         &         &         &         &  (0.003)\\
Constant                      &    1.768&    2.157&    2.125&    2.158&    2.548\\
                              &  (0.036)&  (0.049)&  (0.038)&  (0.049)&  (0.289)\\
Subject FE                    &      Yes&      Yes&      Yes&      Yes&       No\\
Round FE                      &      Yes&      Yes&      Yes&      Yes&      Yes\\
\hline
Observations                  &     2492&     7456&     7456&     7456&     7456\\
\(R^{2}\)                     &     0.41&     0.16&     0.19&     0.16&     0.05\\
\hline\hline
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> mr_reg_results.tex <==
\begin{tabular}{l*{8}{c}}
\toprule
  Dep Var:   &\multicolumn{5}{c}{Sports}  &\multicolumn{2}{c}{Finance} \\ \cmidrule(lr){2-6} \cmidrule(lr){7-8}
 Movement &\multicolumn{1}{c}{Soccer}&\multicolumn{1}{c}{Basketball}&\multicolumn{1}{c}{Baseball}&\multicolumn{1}{c}{Hockey}&\multicolumn{1}{c}{Football} &\multicolumn{1}{c}{Raw} &\multicolumn{1}{c}{Risk-Adj.}\\
\midrule
Uncert.\ Red.\       &           0.839&       0.797&        0.903&        0.987&        0.912&        0.932&        0.903\\
                      &         (0.033)&     (0.024)&      (0.017)&      (0.032)&      (0.016)&      (0.020)&      (0.022)\\
Constant              &          0.0014&      0.0018&       0.0024&       0.0013&       0.0015&       0.0045&       0.0047\\
                      &        (0.0003)&    (0.0003)&     (0.0005)&     (0.0009)&     (0.0002)&     (0.0008)&     (0.0009)\\
\midrule
%$\sqrt{\text{Constant}}$&          0.037&        0.043&        0.049&       0.036&        0.039&        0.067&       0.068\\
$R^2$                   &          0.984&        0.991&        0.996&       0.990&        0.997&        0.991&       0.992\\
Time Chunks         &             12&           12&           12&          12&           12&           16&          16\\
Events                  &          175,026&        48,430&        16,536&       19,445&        3,212&          955&         955\\
Observations            &      4,589,289&      867,567&      166,346&     109,751&       86,193&       27,138&      27,138\\
$p$-val.: $\beta_1=1$     &         0.000&       0.000&       0.000&      0.685&        0.000&        0.046&      0.000\\
$p$-val.: $\beta_0=0$     &         0.000&       0.000&       0.000&      0.162&        0.000&       0.000&      0.000\\
\bottomrule
\end{tabular}



==> mr_reg_resultsMorePeriods.tex <==
\begin{tabular}{l*{8}{c}}
\toprule
  Dep Var:   &\multicolumn{5}{c}{Sports}  &\multicolumn{2}{c}{Finance} \\ \cmidrule(lr){2-6} \cmidrule(lr){7-8}
 Movement &\multicolumn{1}{c}{Soccer}&\multicolumn{1}{c}{Basketball}&\multicolumn{1}{c}{Baseball}&\multicolumn{1}{c}{Hockey}&\multicolumn{1}{c}{Football} &\multicolumn{1}{c}{Raw} &\multicolumn{1}{c}{Risk-Adj.}\\
\midrule
Uncert.\ Red.\       &           0.918&       0.806&        0.889&        0.945&        0.912&        0.670&        0.733\\
                      &         (0.062)&     (0.017)&      (0.019)&      (0.072)&      (0.008)&      (0.051)&      (0.055)\\
Constant              &          0.0009&      0.0018&       0.0026&       0.0018&       0.0015&       0.0065&       0.0060\\
                      &        (0.0003)&    (0.0002)&     (0.0003)&     (0.0010)&     (0.0002)&     (0.0004)&     (0.0004)\\
\midrule
%$\sqrt{\text{Constant}}$&          0.037&        0.043&        0.049&       0.036&        0.039&        0.067&       0.068\\
$R^2$                   &          0.977&        0.985&        0.995&       0.976&        0.995&        0.943&       0.941\\
Time Chunks      &             24&           24&           24&          24&           24&           24&          24\\
Events                  &          175,026&        48,430&        16,536&       19,445&        3,212&          955&         955\\
Observations            &      4,589,289&      867,567&      166,346&     109,751&       86,193&       58,864&      58,864\\
$p$-val.: $\beta_1=1$     &          0.198&       0.000&       0.000&      0.458&        0.000&       0.000&      0.000\\
$p$-val.: $\beta_0=0$     &         0.005&       0.000&       0.000&      0.079&        0.000&       0.000&      0.000\\
\bottomrule
\end{tabular}



==> mr_reg_resultsMorePeriodsGLS.tex <==
\begin{tabular}{l*{8}{c}}
\toprule
  Dep Var:   &\multicolumn{5}{c}{Sports}  &\multicolumn{2}{c}{Finance} \\ \cmidrule(lr){2-6} \cmidrule(lr){7-8}
 Movement &\multicolumn{1}{c}{Soccer}&\multicolumn{1}{c}{Basketball}&\multicolumn{1}{c}{Baseball}&\multicolumn{1}{c}{Hockey}&\multicolumn{1}{c}{Football} &\multicolumn{1}{c}{Raw} &\multicolumn{1}{c}{Risk-Adj.}\\
\midrule
Uncert.\ Red.\       &           1.030&       0.989&        0.925&        0.946&        0.930&        0.800&        0.861\\
                      &         (0.035)&     (0.069)&      (0.019)&      (0.055)&      (0.044)&      (0.068)&      (0.074)\\
Constant              &          0.0004&      0.0007&       0.0020&       0.0015&       0.0013&       0.0055&       0.0049\\
                      &        (0.0002)&    (0.0003)&     (0.0002)&     (0.0007)&     (0.0002)&     (0.0004)&     (0.0004)\\
\midrule
%$\sqrt{\text{Constant}}$&          0.037&        0.043&        0.049&       0.036&        0.039&        0.067&       0.068\\
$R^2$                   &          0.986&        0.927&        0.990&       0.948&        0.976&        0.851&       0.837\\
Time Chunks      &             24&           24&           24&          24&           24&           24&          24\\
Events                  &          175,026&        48,430&        16,536&       19,445&        3,212&          955&         955\\
Observations            &      4,589,289&      867,567&      166,346&     109,751&       86,193&       58,864&      58,864\\
$p$-val.: $\beta_1=1$     &         0.399&       0.879&       0.001&      0.332&        0.124&       0.000&      0.000\\
$p$-val.: $\beta_0=0$     &         0.022&       0.027&       0.000&      0.042&        0.000&       0.000&      0.000\\
\bottomrule
\end{tabular}


